SeaPlace: Process Variation Aware Placement for Reliable Combinational Circuits against SETs and METs

Nowadays nanoscale combinational circuits are facing significant reliability challenges including soft errors and process variations. This paper presents novel process variation-aware placement strategies that include two algorithms to increase the reliability of combinational circuits against both Single Event Transients (SETs) and Multiple Event Transients (METs). The first proposed algorithm is a global placement method (called SeaPlace-G) that places the cells for hardening the circuit against SETs by solving a quadratic formulation. Afterwards, a detailed placement algorithm (named SeaPlace-D) is proposed to increase the circuit reliability against METs by solving a linear programming optimization problem. Experimental results show that SeaPlace-G and SeaPlace-D averagely achieve 41.78% and 32.04% soft error reliability improvement against SET and MET, respectively. Moreover, when SeaPlace-D is followed by SeaPlace-G, MET reduction can be improved by up to 53.3%.

==> Section_Modelling.tex <==
\section{Within-Die  Process Variation Modelling} \label{modelling}
In this section, we intend to present the model used for WID process variation and construct a variation map based on it. WID process variations have two components: Systematic and Random variations. Systematic variations lead to spatial correlation causing that neighbor transistors exhibit similar process parameter values \cite{28}. Differently, random variations result in uncorrelated difference among the process parameters of transistors, even nearby transistors.

In this work, we use VARIUS framework \cite{32} to apply WID variations to process parameters of circuits. In this framework it is supposed that the chip is partitioned into N×N rectangular segments with the same dimensions. In each segment, the process parameter is modeled as a random variable with normal distribution having zero mean and a standard deviation of $\sigma_{sys}$.

VARIUS models the systematic variations with a multivariate normal distribution and uses a spherical structure for modeling the spatial correlation. Its function of correlation is dependent on Euclidean distance between segments.
\begin{equation} \label{eq:1}
Correlation \left(X,\ Y\right)= \rho (r); \quad r= \lvert \vec{X} - \vec{Y} \rvert
\end{equation}
In Eq. \ref{eq:1}, $X$ and $Y$ are two segments and $r$ is their Euclidean distance. In definition of systematic variation, if $r$ is equal to zero, the segments are fully correlated and value of $r$ is one; and if $r$ approaches infinity the segments are fully uncorrelated and $\rho (r)$ is equal to zero. The used spatial correlation is as follows \cite{32}:
\begin{equation} \label{eq:2}
\rho (r) = \left\{
        \begin{array}{ll}
            1 - \frac{3r}{2\phi} + \frac{r^3}{2\phi^3} & \quad r \leq \phi \\
            0 & \quad Otherwise
        \end{array}
    \right.
\end{equation}
where $\phi$ is a parameter to specify the measure of spatial correlation. The limit of function $\rho (r)$ is zero as $r$ approaches . This indicates that the spatial correlation of two segments is constantly decreasing prior to reaching the distance $\phi$ and segments with a distance more than $\phi$ have not any correlation. In the model $\phi$ is expressed as a fraction of the chip’s length.

Channel length $(L_{eff})$ and threshold voltage $(V_{th})$ are two process parameters that are typically considered to be affected by WID variations. In the model of VARIUS \cite{32} there is following relationship between these two parameters:
\begin{equation} \label{eq:3}
L_{eff} = L_{eff}^{n} \left(1 + \frac{V_{th} - V_{th}^{n}}{2V_{th}^{n}} \right)
\end{equation}
where $L_{eff}^{n}$ and $V_{th}^{n}$ are nominal values of $L_{eff}$ and $V_{th}$ respectively. As a result, we only consider the variations in $V_{th}$ in our work, as $L_{eff}$ can be calculated using Eq. \ref{eq:3}.

For constructing a variation map of $V_{th}$, we assume that the chip is partitioned into a N×N grid and run VARIUS with $\mu = 0.22$ \cite{33}, $3\sigma = 55\%$ \cite{33}, N = 300 and correlation distance $\phi=0.5$. The result is a variation map of systematic component of $V_{th}$. In this work, it is supposed that systematic and random components of $\sigma (V_{th})$ are equal; that is $\sigma_{sys} = \sigma_{rand} = \frac{\sigma}{\sqrt{2}}$ \cite{34}. We then generate a N×N matrix of samples from a zero-mean normal distribution with $\sigma_{rand} (V_{th})$. The final $V_{th}$ map is constructed by superposing systematic and random maps segment by segment that is shown in Figure \ref{fig:2}.

\begin{figure}[t]
	\begin{center}
		\includegraphics[width = 0.3\textwidth]{fig/variation_map_ok.png}
		\caption{Systematic $V_{th}$ variation map for a chip with $\Phi=0.5$ ,$\mu=220$,$\sigma=40$, N=300}
	\label{fig:2}
	\end{center}	
\end{figure}

==> ack.tex <==
\section*{Acknowledgment}
The authors would like to thank...

